Overview of the Amphion Toolkit (v0.2)

Amphion is an open-source toolkit for Audio, Music, and Speech Generation, designed to lower the entry barrier for junior researchers and engineers in these fields. It provides a versatile framework that supports a variety of generation tasks and models. In this report, we introduce Amphion v0.2, the second major release developed in 2024. This release features a 100K-hour open-source multilingual dataset, a robust data preparation pipeline, and novel models for tasks such as text-to-speech, audio coding, and voice conversion. Furthermore, the report includes multiple tutorials that guide users through the functionalities and usage of the newly released models.

==> section3_components/visualization.tex <==
\subsection{Visualization} \label{sec:tech_visualization}
\begin{figure*}[htbp]
    \centering
    \includegraphics[width=\textwidth]{section3_components/figs/explainer_system_notes.pdf}
    % \includegraphics[width=0.9\textwidth]{figs/explainer_system.pdf}
    % \includegraphics[scale=0.6]{figs/explainer_system.pdf}
     \vspace{-10pt}
    \caption{
    %\jun{Display this figure in a teaser mode or move it into Section 5.} 
    Amphion v0.2's Visual system for diffusion-based singing voice conversion. The system consists of five views. 
    (A) \textbf{\textit{Metric View}} shows objective evaluation results on the singing voice conversion model, allowing users to interactively explore the performance trend along diffusion steps. (B) \textbf{\textit{Projection View}} aids users in tracking the data patterns of diffusion steps in the embedding space under different input conditions. (C) \textbf{\textit{Step View}} provides users with the visualization of Mel spectrogram and pitch contour at one diffusion step. (D) \textbf{\textit{Comparison View}} facilitates users to compare voice conversion results among different diffusion steps or singers. (E) \textbf{\textit{Control Panel}} enables users to select various comparison modes and choose different source and target singers to visually understand and analyze the model behavior. The red annotations provide explanations for the patterns or components. 
   % \lmxue{upate figure and caption}
     % \vspace{-19pt}
    }
    \label{fig:explainer_system}
\end{figure*}

% Although the diffusion model has shown impressive quality and performance when applied to SVC, our understanding of its internal mechanisms is still limited. 
Visualizing deep learning models is significant for explainable AI systems, and is very educative.
We release a visual analytics system SingVisio~\cite{singvisio} in Amphion v0.2\footnote{\url{https://github.com/open-mmlab/Amphion/tree/main/visualization/SingVisio/webpage}}.
It is designed to interactively explain diffusion models in Singing Voice Conversion(SVC).
% Firstly, the existing diffusion models are still based on \textit{black-box neural networks.} 
Its first benefit is to deepen researchers' comprehension of the diffusion model's operating principles by seeing singing voice conversion through step-by-step denoising. 
Secondly, the SVC conditions, which serve as inputs to the diffusion model, are crucial factors influencing the final conversion results.
Visualizing the diffusion procedure with under different input choices help researchers learn about how to properly choose them.
We follow a procedure in human-computer interaction to develop the Visualization system in Amphion, consisting of the following steps:

\textbf{Step 1: Identifying the Model for Visualization.}
The development of SingVisio began by selecting the core generative model to visualize. The chosen model, DSFF-SVC~\cite{multiple-contents-svc}, is a diffusion-based model specifically tailored for singing voice conversion.

\textbf{Step 2: Task Analysis.}
Through discussions with model builders and researchers, we identified the key requirements, such as \textit{visualizing the classical denoising generation process, comparing results at different diffusion steps, and exploring the influence of content, melody, and singer timbre on the SVC output}.

\textbf{Step 3: Data and Feature Generation.}
We generated the data and features necessary for visualization based on the diffusion model. This included intermediate outputs at each step of the diffusion process and associated metrics, such as signal-to-noise ratios and quality scores. The system was designed to pre-compute these features.

\textbf{Step 4: User Interface Design.}
The web-based user interface was developed using \textit{D3.js}, a powerful JavaScript library for creating dynamic and interactive data visualizations. 

\textbf{Step 5: Iterative Refinement.}
To ensure a seamless user experience, the interface was refined iteratively based on feedback from researchers, practitioners, and novices. Each iteration focused on improving the layout, functionality, and visual clarity of the system to cater to both novice and expert users.

% SingVisio serves as a robust and interactive visual analytics tool, enabling users to explore the intricate workings of diffusion-based models in singing voice conversion. By supporting both foundational understanding and advanced analysis, it addresses the needs of a broad spectrum of users, from beginners to experts.

Fig.~\ref{fig:explainer_system} shows the overview of the system which consists of five front-end components: \textbf{\textit{Control Panel}} allows users to modify mode and choose data for visual analysis; \textbf{\textit{Step View}} provides users with an overview of the diffusion generation process; \textbf{\textit{Comparison View}} makes it easy for users to compare converted results between different conditions; \textbf{\textit{Projection View}} helps users observe the trajectory of diffusion steps with or without conditions; \textbf{\textit{Metric View}} displays objective metrics evaluated on the diffusion-based SVC model, enabling users to interactively examine metric trends across diffusion steps.
% Therefore, a visualization diffusion-based SVC under different diffusion steps and diverse SVC conditions, like varied sources and targets.



==> section4_tutorials/visualization.tex <==
\subsection{Using Amphion Visualization Tool}

% \wcr{brief introduction of SingVisio -> how to prepare data -> how to set up env -> how to run code -> what's the output -> common questions and issues}

\subsubsection{Introduction to SingVisio}
\textit{SingVisio} is a visual analytics tool designed to explain the diffusion model used in singing voice conversion (SVC). It bridges the gap between complex machine learning models and users by providing an intuitive, interactive platform for exploring diffusion-based generation processes. Developed as part of the paper \textit{"SingVisio: Visual Analytics of the Diffusion Model for Singing Voice Conversion"}, this tool offers a web-based user interface and a robust diffusion model back-end.

The system supports five analytical tasks, including step-wise comparisons of diffusion processes and pairwise evaluations of SVC results under varying conditions. The web-based interface, built using \textit{D3.js}, allows users to visualize results in dynamic views. The core diffusion model, \textit{MultipleContentsSVC}, underpins the system’s ability to convert singing voices across different timbres, melodies, and songs with high fidelity.

The online version of SingVisio can be accessed at \url{https://openxlab.org.cn/apps/detail/Amphion/SingVisio}. For implementation details, refer to the source code available for both the front-end visualization and the core generative model.

\paragraph{Tasks Supported in SingVisio}
SingVisio supports five key analytical tasks for evaluating SVC results:

\begin{itemize}
    \item \textbf{T1: Step-wise Diffusion Generation Comparison} - Explore the evolution and quality of converted results at each step of the diffusion process.
    \item \textbf{T2: Step-wise Metric Comparison} - Examine how objective metrics such as Dembed, MCD, and F0CORR vary across diffusion steps.
    \item \textbf{T3: Pair-wise SVC Comparison with Different Target Singers} - Evaluate the effects of converting the same source to different target singers.
    \item \textbf{T4: Pair-wise SVC Comparison with Different Source Singers} - Compare results from converting different source singers to the same target.
    \item \textbf{T5: Pair-wise SVC Comparison with Different Songs} - Investigate the impact of varying source songs on the conversion results.
\end{itemize}

\paragraph{View Design in SingVisio}
The user interface of SingVisio consists of five dynamic views, each supporting a specific aspect of analysis:

\begin{enumerate}
    \item \textbf{Control Panel (View A):} Enables users to adjust display modes and select data for analysis, such as source singers, target singers, and songs.
    \item \textbf{Step View (View B):} Provides a visual representation of the diffusion generation process, allowing users to observe how noise evolves into coherent results.
    \item \textbf{Comparison View (View C):} Facilitates side-by-side comparisons of SVC results under different conditions or steps.
    \item \textbf{Projection View (View D):} Visualizes diffusion step embeddings in a 2D space (e.g., t-SNE) to help users analyze trajectory patterns and clustering.
    \item \textbf{Metric View (View E):} Displays objective metrics, such as timbre similarity and pitch accuracy, evaluated across diffusion steps. Users can interact with metric curves to explore trends and inspect detailed results.
\end{enumerate}

% \subsection{System Installation and Configuration}

\subsubsection{Installation}
\paragraph{Step 1: Install Python and Required Libraries}
Ensure Python 3.10 or higher is installed. Use the following command to verify:
\begin{lstlisting}
python --version
\end{lstlisting}
Install the necessary Python libraries:
\begin{lstlisting}
pip install numpy scikit-learn flask flask_cors gunicorn
\end{lstlisting}

\paragraph{Step 2: Clone the SingVisio Repository}
Clone the repository using Git:
\begin{lstlisting}
git clone <repository-link>
cd SingVisio
\end{lstlisting}

\paragraph{Step 3: Configure Data Paths}
Edit the \texttt{config/default.json} file to specify the paths to your data. For example:
\begin{lstlisting}
{
    "pathData": {
        "<mode_name>": {
            "users": ["basic", "advanced"],
            "multi": ["<id>"],
            "curve": true,
            ...
        }
    }
}
\end{lstlisting}
If hosting data locally, update the \texttt{baseLink} variable in the \texttt{index.html} file on line 15:
\begin{lstlisting}
<script>
    const baseLink = ''; // set to local data path
</script>
\end{lstlisting}

\paragraph{Step 4: Start the Server}
Navigate to the \texttt{webpage} directory and start the server using:
\begin{lstlisting}
cd webpage
gunicorn -w 8 -b 0.0.0.0:8080 server:app
\end{lstlisting}
Access the interface in a browser at \url{http://localhost:8080/}.

\subsubsection{Navigating and Using SingVisio}

\paragraph{Using the Control Panel}
The control panel (View A) is the primary interface for adjusting analysis settings. It provides:
\begin{itemize}
    \item Dropdown menus for selecting display modes, singers, and songs.
    \item A step controller slider to explore results across diffusion steps.
    \item Checkboxes for enabling specific components, such as F0 contours or frequency ranges.
\end{itemize}

\paragraph{Step View and Diffusion Process Visualization}
In the \textbf{Step View (View B)}, users can:
\begin{itemize}
    \item Observe the gradual denoising process in the Mel spectrogram as it transitions from noisy to coherent.
    \item Listen to audio clips at specific steps to perceive quality improvements.
\end{itemize}

\paragraph{Comparing Results with the Comparison View}
The \textbf{Comparison View (View C)} allows:
\begin{itemize}
    \item Side-by-side analysis of audio and spectrograms under different diffusion steps or conditions.
    \item Highlighting differences using color-coded visualizations to identify refined areas.
\end{itemize}

\paragraph{Analyzing Metrics in the Metric View}
The \textbf{Metric View (View E)} supports:
\begin{itemize}
    \item Interactive exploration of metric trends, such as Dembed and FAD, across diffusion steps.
    \item Selection of specific metrics to examine their influence on SVC quality.
\end{itemize}

\paragraph{Advanced Analysis with the Projection View}
In the \textbf{Projection View (View D)}, users can:
\begin{itemize}
    \item Visualize high-dimensional step embeddings using t-SNE projections.
    \item Observe clustering patterns to understand the progression of diffusion steps.
    \item Click on specific points to view corresponding spectrograms and metrics in the Comparison View.
\end{itemize}

\textbf{Troubleshooting and FAQs}
\begin{table}[h!]
\centering
\begin{tabular}{|p{0.3\textwidth}|p{0.3\textwidth}|p{0.3\textwidth}|}
\hline
\textbf{Issue} & \textbf{Cause} & \textbf{Solution} \\
\hline
Webpage not loading & Server not running or configuration errors & Verify server status and \texttt{config/default.json} paths. \\
\hline
Metrics missing & Invalid or missing dataset configuration & Update \texttt{config/default.json} with valid data paths. \\
\hline
Audio playback fails & Missing audio files or browser issues & Check audio paths and ensure browser compatibility. \\
\hline
Projection View anomalies & Poor embedding parameters & Adjust t-SNE parameters or preprocess data. \\
\hline
\end{tabular}
\caption{Common issues and solutions for SingVisio.}
\end{table}

==> section6_conclusion/visualiazation.tex <==
\subsection{Visualization}
To evaluate Amphion v0.2's Visualization system, we ask 23 Amphion users to fill a questionnaire of 15 questions covering four aspects (A1-A4), including explainability, functionality, effectiveness, and usability of the SingVisio system in Amphion. 
Each question has a scale ranging from 1 to 5, i.e., strongly disagree (1), disagree (2), neutral (3), agree (4), and strongly agree (5), and higher scores indicate positive impressions. 
Detailed results for each dimension and question are presented in Fig.~\ref{fig:sbj}.
The assessment results yield an extraordinary average score of 4.67 (\(\sigma=0.02\)).
Notably, our system achieved the highest score in analysis functionality (\(\mu = 4.76\), \(\sigma=0.13\)) and also performed well in effectiveness  (\(\mu = 4.74\), \(\sigma=0.0\)). 
\begin{figure*}[h!]
    \centering
    \includegraphics[width=\textwidth]{section5_experiments/figs/sbj.pdf}
    \vspace{-10pt}
    \caption{Rating scores of user impressions to Amphion v0.2's SingVisio visualization module. A1-A4 represents the four aspects, including explainability, functionality, effectiveness, and usability. S1-S15 denotes 15 subjective questions. The rightmost value shows the mean ± standard deviation for each question.} 
    % The details of 15 subjective questions are presented in ~\ref{app:questions}. 
    \label{fig:sbj}
     % \vspace{-19pt}
\end{figure*}
